On the Difficulty of Unbiased Alpha Divergence Minimization

Several approximate inference algorithms have been proposed to minimize an alpha-divergence between an approximating distribution and a target distribution. Many of these algorithms introduce bias, the magnitude of which becomes problematic in high dimensions. Other algorithms are unbiased. These often seem to suffer from high variance, but little is rigorously known. In this work we study unbiased methods for alpha-divergence minimization through the Signal-to-Noise Ratio (SNR) of the gradient estimator. We study several representative scenarios where strong analytical results are possible, such as fully-factorized or Gaussian distributions. We find that when alpha is not zero, the SNR worsens exponentially in the dimensionality of the problem. This casts doubt on the practicality of these methods. We empirically confirm these theoretical results.

==> sections/intro.tex <==
% !TEX root = ../main.tex

\section{Introduction}

Variational Inference (VI) typically minimizes the ``exclusive'' KL-divergence between an approximating distribution $q_w(z)$ and a target distribution $p(z)$, $\KL(q_w||p)$ \citep{jordan1999introduction, blei2017variational, zhang2017advances}. While computationally convenient, the use of this objective may lead to distributions $q_w$ with undesirable statistical properties. For instance, it leads to distributions $q_w$ that underestimate the variance of $p$ \citep{minka2005divergence}. To avoid these issues one could consider minimizing a different objective. An alternative is the $\alpha$-divergence \citep{amari1985differential},

\small
\begin{equation}
D_\alpha(p||q_w) = \frac{1}{\alpha(\alpha - 1)} \E_{q_w}\left[ \left(\frac{p(z)}{q_w(z)}\right)^\alpha - 1 \right],\quad \alpha \in \mathbb{R} \setminus \{0, 1\}. \label{eq:obj_a}
\end{equation}
\normalsize

This divergence is indexed by the parameter $\alpha$, which determines its properties. For $\alpha \gg 0$, the divergence will penalize distributions $q_w$ that place no mass in regions where $p$ does, penalizing under-dispersion \citep{minka2005divergence, hernandez2016black}. Therefore, minimizing $D_\alpha(p||q_w)$ for $\alpha \gg 0$ will lead to distributions $q_w$ that are over-dispersed with respect to $p$. The $\alpha$-divergence recovers several well known divergences for different values of $\alpha$ \citep{amari2010families}: the $\chi^2$-divergence for $\alpha = 2$, and the Hellinger distance for $\alpha = 0.5$. For $\alpha = 0$ and $\alpha = 1$ the divergence is defined as the limits $\alpha \rightarrow 0$ and $\alpha \rightarrow 1$, which result in $\KL(q_w||p)$ and $\KL(p||q_w)$, respectively.

Several algorithms have been developed with the goal of minimizing $\alpha$-divergences. These can be classified into two broad groups: biased methods \citep{powerEP, hernandez2016black, renyiVI, regli2018alpha} and unbiased methods \citep{kuleshov2017neural, dieng2017chivi}. Methods in the former group do not exactly minimize an $\alpha$-divergence, they either minimize local surrogates and/or use biased gradient estimators. On the other hand, unbiased methods attempt to run SGD with unbiased estimators of $\nabla_w D_\alpha(p||q_w)$. While \cite{dieng2017chivi} and \cite{kuleshov2017neural} show some positive empirical results for unbiased methods, they both stress that the gradient exhibits high variance. This causes difficulties scaling these methods to high dimensional models.

There are two open questions regarding these methods. First, how much bias do biased methods have? Second, how much variance do unbiased methods have? Currently, it is unclear when these methods will succeed, or how the bias and variance depends on $\alpha$ or the dimensionality of $z$.

In this work we address the second question. We focus on \textit{unbiased} methods for $\alpha$-divergence minimization, with the goal of understanding how these methods scale to problems of large dimensionality for different values of $\alpha$. Our analysis includes a rigorous study of the properties of the unbiased gradient estimators used and empirical results on illustrative scenarios. The main conclusion is as follows: methods based on unbiased estimates of $\nabla_w D_\alpha(p||q_w)$ will not scale to high dimensional models for values of $\alpha \neq 0$. This is not always due to high variance gradients, but due to an extremely low Signal-to-Noise ratio (SNR).

In Section \ref{sec:motiv} we present two gradient estimators used by unbiased methods, one obtained using reparameterization, and a novel one obtained by applying ``double'' reparameterization. We also present an empirical evaluation that shows that, even in a very simple scenario, these methods do not seem scale to problems of moderately high dimension ($d \approx 100$), nor to moderately large values of $\alpha$ ($\alpha \approx 0.4$). Curiously, optimization fails even in some cases where the gradient estimator has provably low variance. Instead, we propose that this failure is best explained by the estimator's SNR. In Section \ref{sec:NSR} we analyze SNR for three scenarios for $p$ and $q_w$: arbitrary fully-factorized distributions, fully-factorized Gaussians, and Gaussians with arbitrary full-rank covariances. We give exact results for the SNR in each of these three cases. We see that for \textit{any} $\alpha \neq 0$, under mild assumptions, the SNR decreases \textit{exponentially} in the dimensionality of the problem. Thus, even in these simple scenarios, unbiased methods will scale extremely poorly to high dimensions. Finally, in Section \ref{sec:exps} we test some more general scenarios, and confirm that the same phenomena seems to occur.

